Estimating galaxy masses from kinematics of globular cluster systems: a new method based on deep learning

We present a new method by which the total masses of galaxies including dark matter can be estimated from the kinematics of their globular cluster systems (GCSs). In the proposed method, we apply the convolutional neural networks (CNNs) to the two-dimensional (2D) maps of line-of-sight-velocities ($V$) and velocity dispersions ($\sigma$) of GCSs predicted from numerical simulations of disk and elliptical galaxies. In this method, we first train the CNN using either only a larger number ($\sim 200,000$) of the synthesized 2D maps of $\sigma$ ("one-channel") or those of both $\sigma$ and $V$ ("two-channel"). Then we use the CNN to predict the total masses of galaxies (i.e., test the CNN) for the totally unknown dataset that is not used in training the CNN. The principal results show that overall accuracy for one-channel and two-channel data is 97.6\% and 97.8\% respectively, which suggests that the new method is promising. The mean absolute errors (MAEs) for one-channel and two-channel data are 0.288 and 0.275 respectively, and the value of root mean square errors (RMSEs) are 0.539 and 0.51 for one-channel and two-channel respectively. These smaller MAEs and RMSEs for two-channel data (i.e., better performance) suggest that the new method can properly consider the global rotation of GCSs in the mass estimation. We also applied our proposed method to real data collected from observations of NGC 3115 to compare the total mass predicted by our proposed method and other popular methods from the literature.

==> table <==
%%% TABLE 1
\begin{table}
\centering
\begin{minipage}{80mm}
\caption{Description of the basic parameter values
for the fiducial model for merging of two disk galaxies
}
\begin{tabular}{ll}
{Physical properties}
& {Parameter values}\\
Total halo mass (galaxy)
& $M_{\rm dm}=1.0 \times 10^{12} {\rm M}_{\odot}$  \\
DM structure (galaxy)
& NFW profile \\
Galaxy virial radius (galaxy)
&  $R_{\rm vir}=245$ kpc  \\
$c$ parameter of galaxy halo
&  $c=10$  \\
Number of GCs in a GCS & $N_{\rm gc}=200$     \\
Rotational energy fraction of a GCS & $f_{\rm rot}=0.0$     \\
Stellar disk  mass & $M_{\rm s}=6.0 \times 10^{10} {\rm M}_{\odot}$     \\
Stellar disk size & $R_{\rm s}=17.5$ kpc \\
Gas disk size & $R_{\rm g}=17.5$ kpc \\
Disk scale length & $R_{0}=3.5$ kpc \\
Bulge mass &   $M_{\rm b}=10^{10} {\rm M}_{\odot}$  \\
Bulge size  & $R_{\rm b}=3.5$ kpc \\
Mass resolution & $5.0 \times 10^4 {\rm M}_{\odot}$ \\
Size resolution & 175 pc \\
Mass-ratio of two spirals in a merger & 1.0 \\
Initial distance of two spirals in a merger & 140 kpc \\
Velocity factor of a merger  & $f_{\rm v}=0.45$  \\
Star formation  & Not included \\
Chemical  evolution  &  Not included \\
Dust  evolution  &  Not included \\
\end{tabular}
\end{minipage}
\end{table}

